Analyzing Individual Proofs as the Basis of Interoperability between Proof Systems

We describe the first results of a project of analyzing in which theories formal proofs can be ex- pressed. We use this analysis as the basis of interoperability between proof systems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{3}
\providecommand{\publicationstatus}{C. Dubois and B. Woltzenlogel Paleo (Eds.): Fifth Workshop on \\
Proof eXchange for Theorem Proving (PxTP 2017)\\
EPTCS 262, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.262.1}{10.4204/EPTCS.262.1}}

